KVC-onGoing: Keystroke Verification Challenge

This article presents the Keystroke Verification Challenge - onGoing (KVC-onGoing), on which researchers can easily benchmark their systems in a common platform using large-scale public databases, the Aalto University Keystroke databases, and a standard experimental protocol. The keystroke data consist of tweet-long sequences of variable transcript text from over 185,000 subjects, acquired through desktop and mobile keyboards simulating real-life conditions. The results on the evaluation set of KVC-onGoing have proved the high discriminative power of keystroke dynamics, reaching values as low as 3.33% of Equal Error Rate (EER) and 11.96% of False Non-Match Rate (FNMR) @1% False Match Rate (FMR) in the desktop scenario, and 3.61% of EER and 17.44% of FNMR @1% at FMR in the mobile scenario, significantly improving previous state-of-the-art results. Concerning demographic fairness, the analyzed scores reflect the subjects' age and gender to various extents, not negligible in a few cases. The framework runs on CodaLab.

==> old_7_Experimental_Protocol.tex <==
\subsection{Evaluation of Privacy-Enhancing Input Features}
\label{subsec:evaluation}

The two biometric systems considered, TypeNet and TypeFormer, take as input the same set of features extracted from the raw data (Unix timestamps of the actions of pressing and releasing a key), which include:
\begin{itemize}
    \item[\textit{(i)}] Hold Time (HT): time interval between the release and press instants of a given key, expressed in seconds.
    \item[\textit{(ii)}] Inter-Press Time (IPT): time interval between two consecutive press actions, expressed in seconds.
    \item[\textit{(ii)}] Inter-Release Time (IRT): time interval between two consecutive release actions, expressed in seconds.
    \item[\textit{(iv)}] Inter-Key Time (IKT): time interval between a release and the following press action, expressed in seconds.
    \item[\textit{(v)}] ASCII code (ASCII), normalized by dividing it by 255.
\end{itemize}
Such features are graphically represented in black in Fig. \ref{fig:features}. Input features \textit{(i)}-\textit{(iv)} are useful to capture the typing behavior of the user in the time-domain, whereas the ASCII code \textit{(v)} describes the spatial relations due to the location of the key pressed on the keyboard layout. However, although handled in compliance with sensitive data protection regulations \cite{GDPR2016a}, the acquisition and processing of the ASCII codes inevitably reveals the content of the text, putting at risk the privacy of the users. Consequently, in this experiment, we strive to remove the ASCII code information in order to make the system content-agnostic, and consequently more privacy preserving. The sets of experiments run can be summarized as follows:
\begin{itemize}
    \item[1.] First, to evaluate and compare TypeNet and TypeFormer, we consider their original set of features (the experiment is named \textit{5F}, where ``\textit{F}'' stands for ``features''), marked in black in Fig. \ref{fig:features}.
    \item[2.] Then to quantify the importance of the ASCII code information, we remove the ASCII code information from the original set of features (experiment \textit{4F}).
    \item[3.] We consider an extended set of time-domain features. Several studies have in fact shown the usefulness of considering groups of keys typed such as digraphs, trigraphs, and \textit{n}-graphs \cite{9853506}. By considering not only adjacent keys, but groups of three keys (Fig. \ref{fig:features}, in red and blue), we obtain a set of 10 features (experiment \textit{10F}): 
    \begin{equation*}
        [\textrm{HT}, \textrm{IPT}, \textrm{IRT}, \textrm{IKT}, \textrm{IPT2}, \textrm{IRT2}, \textrm{IKT2},
    \end{equation*}
    \begin{equation*}
        \textrm{IPT3}, \textrm{IRT3}, \textrm{IKT3}]
    \end{equation*}

    \item[4.] We consider the extended set of time-domain features, together with the ASCII code (experiment \textit{11F}).
\end{itemize}
In each case, the deep learning models are trained from scratch.
% 
% We designed four experiments per model in order to assess the performance of different set of features: \textit{(i)} original set of features (\textit{5F}), original set of features without ASCII (\textit{4F}), proposed set of features (\textit{10F}), proposed set of features plus ASCII (\textit{11F}).  

\begin{figure}
\centering
  \centering
  \includegraphics[width=\linewidth]{images/features.pdf}
\caption{\footnotesize A diagram representing the initial feature extraction process for the time instant $t = 0$. HT = Hold Time; IPT = Inter-Press Time; IRT = Inter-Release Time; IKT  = Inter-Key Time; IPT2 = Inter-Press Time with second following key; IRT2 = Inter-Release Time with second following key; IKT2  = Inter-Key Time with second following key; IPT3 = Inter-Press Time with third following key; IRT3 = Inter-Release Time with third following key; IKT3  = Inter-Key Time with third following key.}
\label{fig:features}
\end{figure}

\subsection{Model Training}
The training of both models takes place on the KVC development set considering identical settings to those described in their respective papers. The only differences are related to the division into training and validation sets. For TypeNet, we consider a subset of 400 subjects to validate the model at the end of each training epoch in terms of average EER per subject. This choice is justified by the experimental protocol followed in \cite{typenet}. For TypeFormer, we consider an 80\%-20\% train-validation division of the KVC development set, and we adopt the global EER as validation metric. According to these validation metrics, the best-performing epoch model is saved in each case.



